GenURL: A General Framework for Unsupervised Representation Learning

Unsupervised representation learning (URL), which learns compact embeddings of high-dimensional data without supervision, has made remarkable progress recently. However, the development of URLs for different requirements is independent, which limits the generalization of the algorithms, especially prohibitive as the number of tasks grows. For example, dimension reduction methods, t-SNE, and UMAP optimize pair-wise data relationships by preserving the global geometric structure, while self-supervised learning, SimCLR, and BYOL focus on mining the local statistics of instances under specific augmentations. To address this dilemma, we summarize and propose a unified similarity-based URL framework, GenURL, which can smoothly adapt to various URL tasks. In this paper, we regard URL tasks as different implicit constraints on the data geometric structure that help to seek optimal low-dimensional representations that boil down to data structural modeling (DSM) and low-dimensional transformation (LDT). Specifically, DMS provides a structure-based submodule to describe the global structures, and LDT learns compact low-dimensional embeddings with given pretext tasks. Moreover, an objective function, General Kullback-Leibler divergence (GKL), is proposed to connect DMS and LDT naturally. Comprehensive experiments demonstrate that GenURL achieves consistent state-of-the-art performance in self-supervised visual learning, unsupervised knowledge distillation (KD), graph embeddings (GE), and dimension reduction.

==> tables/Tab_app_ablation_ssl.tex <==

\begin{table}[H]
\centering
\resizebox{.95\columnwidth}{!}{
    \begin{tabular}{lccc}
    \toprule
    Method         & batch      & 400ep             & 800ep        \\
                   & size       & Top1, Top 5       & Top1, Top 5  \\ \hline
    SimCLR         & 256        & 82.90, 99.26      & 86.61, 99.30 \\
    SimCLR         & 4096       & 86.92, 99.41      & 89.68, 99.66 \\
    MoCo.v2        & 256        & 84.89, 99.41      & 89.58, 99.30 \\
    MoCo.v2        & 1024       & 84.21, 98.30      & 88.95, 99.14 \\
    GenURL (100\%) & 256        & \bf{88.35, 99.25} & \bf{90.82, 99.41} \\
    GenURL (75\%)  & 256        & 87.86, 99.73      & 89.82, 99.26 \\
    GenURL (50\%)  & 256        & 86.44, 99.16      & 89.05, 99.10 \\
    GenURL (25\%)  & 256        & 85.29, 98.79      & 87.64, 99.57 \\
    \bottomrule
    \end{tabular}}
    \caption{Ablation of convergence speed of GenURL and CL methods on STL-10.}
    \label{tab:app_ablation}
\end{table}


==> tables/Tab_app_ge_dataset.tex <==

\begin{table}[H]
\centering
\resizebox{.90\columnwidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule
             & Nodes  & Features & Edges  & Class   & $\nu_{Z}$ & $\alpha_2$ \\ \hline
    CORA     & 2,708  & 1,433    & 5,429  & 7       & 0.001     & 1.0        \\
    CiteSeer & 3,327  & 3,703    & 4,732  & 6       & 0.005     & 0.5        \\
    PubMed   & 19,717 & 500      & 44,338 & 3       & 0.003     & 50         \\
    \bottomrule
    \end{tabular}}
    \caption{Basic information and GenURL hyper-parameters of graph datasets.}
    \label{tab:app_ge_dataset}
\end{table}


==> tables/Tab_app_img_dataset.tex <==

\begin{table}[H]
\centering
\resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{lccccc}
    \toprule
    Dataset       & Tasks   & Train   & Test & Resolution     & Class \\ \hline
    MNIST         & DR      & 50k     & 10k  & 28$\times$28   & 10      \\
    FMNIST        & DR      & 50k     & 10k  & 28$\times$28   & 10      \\
    CIFAR-10      & SSL     & 50k     & 10k  & 32$\times$32   & 10      \\
    CIFAR-100     & SSL     & 50k     & 10k  & 32$\times$32   & 100     \\
    STL-10        & SSL, KD & 5k+100k & 8k   & 96$\times$96   & 10      \\
    Tiny-ImageNet & SSL     & 100k    & 10k  & 64$\times$64   & 200     \\
    ImageNet-1k   & SSL     & 1.28M   & 5k   & 224$\times$224 & 1k      \\
    \bottomrule
    \end{tabular}}
    \caption{Basic information of image datasets.}
    \label{tab:app_img_dataset}
\end{table}

